Applications of single-photon technology

This doctoral dissertation deals with the subject of single-photon technology applications. Particular emphasis was placed on the use of single-photon sources in quantum communication, metrology, and further development of quantum computers. At the beginning of this thesis, the development history of cryptography is described, starting from steganography and ending with quantum key distribution protocols. Later, the key elements of the quantum network, such as end nodes and transmission channels, are presented. Various types of sources and single-photon detectors are discussed. Methods for amplifying the signal and correcting errors that occur during transmission are also mentioned. In the further part of this thesis, two examples of single-photon sources are described, along with their experimental implementation. These sources are based on the nonlinear spontaneous parametric down-conversion (SPDC) process, which has also been described in detail. Parameters that specify the quality of a single-photon source (such as conversion efficiency, phase-matching conditions, singleness and photonic density matrix) are also characterized, both mathematically and experimentally. Furthermore, this doctoral dissertation consists of definitions and elaborated descriptions of quantum optical phenomena, which should be useful for those who are not yet familiar with the subject of single-photon sources and their applications or just start their work in this field.

==> ch3s3.tex <==
\subsection{Source No 3 -- infrared photon triplets}
\label{sec:ch3-3ph}

\begin{figure}[t]
\centering
\includegraphics[width=0.7\linewidth]{pic/cp3source.jpg}
\caption{Scheme of photon triplet source. Symbols: S1 -- pump laser source no. 1 (pulsed, Chameleon Coherent Inc.), S2 -- pump laser source no. 2 (continuous wave, ECD-X MSquare), M -- silver mirror (Thorlabs PF10-03-P01), DM -- dichroic mirror (Semrock FF605-Di02), L1 -- plano-convex lens (focal length $f=7.5cm$), BIBO -- bismuth triborate crystal, L2 -- plano-convex lens (focal length $f=10cm$), M -- gold mirror (Thorlabs PF10-03-M01), C -- collimation package (Throlabs CFC-11X-C), SMF -- single mode fiber, SSPD -- superconducting single-photon detector.}
\label{pic:s3}
\end{figure}
\FloatBarrier
